A numerically stable communication-avoiding s-step GMRES algorithm

Krylov subspace methods are extensively used in scientific computing to solve large-scale linear systems. However, the performance of these iterative Krylov solvers on modern supercomputers is limited by expensive communication costs. The $s$-step strategy generates a series of $s$ Krylov vectors at a time to avoid communication. Asymptotically, the $s$-step approach can reduce communication latency by a factor of $s$. Unfortunately, due to finite-precision implementation, the step size has to be kept small for stability. In this work, we tackle the numerical instabilities encountered in the $s$-step GMRES algorithm. By choosing an appropriate polynomial basis and block orthogonalization schemes, we construct a communication avoiding $s$-step GMRES algorithm that automatically selects the optimal step size to ensure numerical stability. To further maximize communication savings, we introduce scaled Newton polynomials that can increase the step size $s$ to a few hundreds for many problems. An initial step size estimator is also developed to efficiently choose the optimal step size for stability. The guaranteed stability of the proposed algorithm is demonstrated using numerical experiments. In the process, we also evaluate how the choice of polynomial and preconditioning affects the stability limit of the algorithm. Finally, we show parallel scalability on more than 114,000 cores in a distributed-memory setting. Perfectly linear scaling has been observed in both strong and weak scaling studies with negligible communication costs.

==> Review/cover_letter.tex <==
\newpage
\noindent Title: A NUMERICALLY STABLE COMMUNICATION AVOIDING S-STEP GMRES ALGORITHM

\noindent Journal: SIAM Journal on Matrix Analysis and Applications (SIMAX)

\noindent Manuscript Number: \#M157710

\noindent Date: \today

\vspace{0.2in}

\noindent Dear Editor and Reviewers,

\vspace{0.2in}
We would like to express our sincere gratitude to the Editor and the reviewers for their invaluable feedback and insightful comments on our manuscript, "A NUMERICALLY STABLE COMMUNICATION AVOIDING S-STEP
GMRES ALGORITHM" (Manuscript Number: \#M157710). We appreciate the time and effort devoted to the peer review process, and we have carefully considered each of the reviewers' comments in preparing this revised version of our manuscript. 

We would also like to extend our sincere appreciation to the Editor for graciously granting extensions to the submission deadlines. This extension has allowed us to regain access to the same cluster used in the original manuscript and given us valuable additional time to enhance the quality of our manuscript. We are genuinely thankful for this considerate accommodation.

Herein, we present our response to the comments provided by the reviewers. Since both reviewers have shared similar comments on benchmarking our algorithm in parallel settings, we would like to address that aspect first to both reviewers. Subsequently, we will provide point-to-point response to individual comments from each reviewer.

We submit this response and the revised manuscript for your consideration and look forward to any further guidance from the Editor and reviewers.

\vspace{0.2in}
Best regards,

\vspace{0.2in}

Zan Xu (Corresponding Author)

Stanford University


==> Review/review.tex <==
\newpage
\section*{Response to both reviewers on benchmarking against other algorithms}
Both reviewers have indicated interests in seeing comparisons of the proposed algorithm, adaptive s-step GMRES, against other existing GMRES algorithms that are not MGS-based. Reviewer \#1 is interested in seeing comparison against CGS2-GMRES and Reviewer \#2 is interested in seeing comparison against TSQR-based s-step GMRES algorithm. We agree with both reviewers that MGS-GMRES is inherently not scalable on large-scale parallel computing architectures. Comparing with a scalable variant would make the comparison more meaningful and rigorous. Since both reviewers have similar requests, we would like to address to both reviewers here regarding comparison against other GMRES algorithms. 

In the manuscript, we have included a significant amount of additional results and rewritten a significant portion of the text in \Cref{sec:scalability}. However, the general observation and conclusions drawn still align with the original manuscript. Here, we would like to highlight the main changes introduced in this manuscript, explain reasons for those changes and highlight the key results.

\begin{itemize}
    \item \textbf{Addition of two more algorithms for comparison} First of all, we took suggestions from both reviewers and included two more algorithms to compare against for parallel testing. In total, we compare four different GMRES algorithms in our weak scaling and strong scaling results: (1) MGS-GMRES: the standard GMRES algorithm based on Modified Gram-Schmidt. (2) CGS2-GMRES: the GMRES algorithm based on Classical Gram-Schmidt with re-orthogonalization. This variant uses CGS2 for orthogonalization which is numerically stable and has better parallel performance. The number of global reductions is constant (three, to be exact) at each iteration. (3) BCGS2-TSQR s-step GMRES: a BCGS2-TSQR based s-step GMRES algorithm where BCGS2 is used as the inter-orthogonalization scheme and TSQR is used as the intra-orthogonalization scheme. (4) Adaptive s-step GMRES: the algorithm proposed in this work (\Cref{alg:adaptsgmres}).
    The first two algorithms are column-wise GMRES algorithms where each iteration works on only one additional Krylov basis vector whereas the last two algorithms are s-step GMRES algorithms where each iteration works on a block of multiple Krylov basis vectors. We would like to highlight that the difference between (3) and (4) is in the intra-orthogonalization scheme. We have included a paragraph in \Cref{sec:scalability} to elaborate on the differences among various GMRES variants. 
    
    \item \textbf{Change in software} There is a change in the software used in all parallel performance tests. The results in the previous version of manuscript was generated using a code written in C++ and the matrix/vector operations were implemented through the Eigen library at version 3.4.0. The C++ code was compiled using Intel compiler 19.1.1 with MKL as the backend for math kernels. Intel MPI 19.0.9 was used for communication. In this revised manuscript, we replace Eigen with PETSc for all matrix operations. The main reason for this change is because of the availability of the TSQR algorithm in PETSc/SLEPc. TSQR algorithm is well-established in literature. However, its software implementation, particularly the parallel version, requires custom communication patterns/trees/maps for efficient reduction-like communication and it is non-trivial to implement them efficiently, especially when the number of MPI ranks is not powers-of-two. Therefore, we want to use a publicly available TSQR algorithm in credible open-source libraries for reproducibility. In this work, we chose the parallel TSQR algorithm in SLEPc, which is based on PETSc. For example, see \href{https://slepc.upv.es/documentation/current/docs/manualpages/BV/BVOrthogBlockType.html#BVOrthogBlockType}{SLEPC BV Orthogonalization Block Types} here. 
    To make fair comparisons, it is best to have all other GMRES variants implemented with the same backend for matrix/vector operations. Therefore, we refactored all of our code. All parallel results in this revised manuscript are generated using the refactored C++ code with PETSc 3.20, SLEPc 3.20 for matrix/vector operations.
    
    During refactoring, we have also upgraded the compiler to Intel oneAPI compiler 23.1.0 to leverage on any recent compiler optimizations (Intel MPI is upgraded to 21.9.0 as well). Based on our experience, the new compiler does seem to improve the performance significantly (see the next point).
    
    All tests were conducted on a cluster equipped with Intel Xeon(R) Platinum 8280 CPUs @ 2.70GHz. All nodes have 56 cores per node and are interconnected via Mellanox Infiniband, HDR-100. The hardware used in this revised manuscript is the same as the previous manuscript.

    \item \textbf{Changes in results with respect to the previous manuscript} Due to the change in the software stack and code refactorization, we re-ran all scaling results (for MGS-GMRES and Adaptive s-step GMRES) to make sure they represent a fair comparison with the newly-added algorithms (CGS2-GMRES, BCGS2-TSQR-GMRES). However, if one were to compare the results for MGS-GMRES and Adaptive s-step GMRES in this revised manuscript against those in the previous manuscript, there will be noticeable performance differences in some mathematical operations due to software changes. Here, we would like to account for how MGS-GMRES and Adaptive GMRES results changed from the initial manuscript to the current revised manuscript, in order to justify the credibility of our new set of results.
    
    \begin{figure}[ht]
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        width=.6\textwidth,
        height=.4\textwidth,
        % bar width=.2cm,
        stack negative=separate,
        ybar stacked,
        xmin=0.5,
        xmax=3.5,
        ymin=-0.1,
        ymax=.4,
        xtick={1,2,3},
        xticklabels={Ver. 1, Ver. 2, Ver. 3$^*$},
        ylabel={time (s)},
        ymajorgrids=true,  
        yminorgrids=true,   
        % minor y tick num=1,
        legend pos=outer north east,
        % legend columns=4,
        % legend style={at={(0.5,1.22)}, anchor=north},
        % ytick={-0.2, 0, 0.2, 0.4, 0.6, 0.8, 1.0},
        % yticklabels={0.2, 0, 0.2, 0.4, 0.6, 0.8, 1.0},
    ]
    \addplot +[draw=black,
    color=hcblue,
    fill opacity=0.8,
    bar shift=-.2cm] table [x=index,y=SpMV_GMRES] {Review/comp.dat};
    \addplot +[draw=black,
    color=hcgreen,
    fill opacity=0.8,
    bar shift=-.2cm] table [x=index,y=Ortho_GMRES] {Review/comp.dat};
    \addplot +[draw=black,
    color=black,
    fill opacity=0.8,
    bar shift=-.2cm] table [x=index,y=Ortho_comm_GMRES] {Review/comp.dat};
    \addplot +[draw=black,
    color=hcred,
    fill opacity=0.8,
    bar shift=-.2cm] table [x=index,y=Other_GMRES] {Review/comp.dat};
    \legend{SpMV, Ortho. (comp), Ortho. (comm), Other};
    \end{axis}
    \begin{axis}[
        width=.6\textwidth,
        height=.4\textwidth,
        % bar width=.2cm,
        stack negative=separate,
        ybar stacked,
        xmin=0.5,
        xmax=3.5,
        ymin=-0.1,
        ymax=.4,
        hide axis,
    ]
    \addplot +[draw=black,
    color=hcblue,
    fill opacity=0.8,
    bar shift=.2cm] table [x=index,y=SpMV_SGMRES] {Review/comp.dat};
    \addplot +[draw=black,
    color=hcgreen,
    fill opacity=0.8,
    bar shift=.2cm] table [x=index,y=Ortho_SGMRES] {Review/comp.dat};
    \addplot +[draw=black,
    color=black,
    fill opacity=0.8,
    bar shift=.2cm] table [x=index,y=Ortho_comm_SGMRES] {Review/comp.dat};
    \addplot +[draw=black,
    color=hcred,
    fill opacity=0.8,
    bar shift=.2cm] table [x=index,y=Other_SGMRES] {Review/comp.dat};
    \end{axis}
    \end{tikzpicture}
    \caption{Timing breakdown for a 1M size 3D Laplace matrix running one a single node. MGS-GMRES is on the left and Adaptive s-step GMRES is on the right. Ver. 1: Original code in the previous manuscript (Eigen library, Intel compiler 19.1.1, Intel MPI 19.0.9). Ver. 2: Original code but compiler with Intel compiler 23.1.0 and Intel MPI 21.9.0. Ver. 3: Refactored code (PETSc library, Intel compiler 23.1.0 and Intel MPI 21.9.0). }
    \label{fig:revision}
\end{figure}

    In \Cref{fig:revision}, we use the same matrix problem (1M Laplace matrix on a single node) and compare three different versions of the code. The first version was based on Eigen library with Intel compiler version 19.1.1 and was used in the previous manuscript. This serves as a baseline for comparison across code versions. The second version uses the same source code, but compiled with an upgraded Intel compiler at version 23.1.0. As seen in the figure, there is a significant speedup in the computation of orthogonalization schemes for the adaptive s-step GMRES algorithm. The MGS orthogonalization stays relatively the same. Note that the orthogonalization in s-step GMRES consists mainly of BLAS-3 kernels whereas MGS uses BLAS-1 kernels. This means that the upgraded Intel compiler (with upgraded built-in MKL) is able to perform more optimizations for BLAS-3 kernels.

    Version 3 is a refactored code that is based on PETSc library, compiled with Intel 23.1.0. The timing breakdown indicates that using PETSc library allows for further optimizations in math kernels. Specifically, speedup is observed for the orthogonalization scheme based on BLAS-3 kernels and the SpMV kernels. 

    Overall, we see significant speedup using the new compiler with refactored code based on PETSc. We would like to highlight that this does not affect the general trend of scaling results, thus it does not contradict with any observation or conclusion in this work. As shown in \Cref{fig:weakscaling} and \Cref{fig:weakscaling_pc}, scalability of the kernel and the overall algorithm is still observed. We can even argue that this speedup in orthogonalization step due to compiler/backend change aligns with the objective of this work, which is to avoid communication, but at an intra-node level. As our algorithm relies on BLAS-3 kernels, more aggressive compiler optimizations and well-implemented PETSc backends can exploit various levels of cache to reduce communication costs associated with data movement across different levels of cache memory, giving rise to more performant results in a single node.
    
    \item Since the time taken for the orthogonalization step in adaptive s-step GMRES is on the order of 0.01s, to mitigate profiling overheads, we increased the size of the weak scaling test matrix from 1M to 8M on a single node. We also included an additional set of experiments at 2048 nodes (114,688 cores). In other words, the matrix size varies from 8M to 16B on 1 to 2048 nodes, instead of the previous configuration with 1M to 256M on 1 to 256 nodes. Please see \Cref{sec:weakscaling} and \Cref{fig:weakscaling_pc} for more details. The vast difference in orthogonalization step between our proposed algorithm and other GMRES variants highlights the benefit of using BCGS2+Partial CholQR for avoiding communication at the intra-node level and at the inter-node level.
\end{itemize}

We hope these points could convince the reviewers that we have thoroughly prepared the additional benchmarking results as requested, and the changes in results are academically sound and credible. For detailed discussion of the benchmarking results among various GMRES variants, please refer to the added text in \Cref{sec:scalability}. Again, we genuinely appreciate the feedback from both reviewers and we completely agree adding these tests does make this manuscript more rigorous and complete.



==> Review/reviewer1.tex <==
\newpage
\section*{Response to reviewer \#1}
\rpy{(Responses are highlighted in red. Corresponding code changes are highlighted in red as well in the manuscript.)}

\subsection*{Major comments}
\paragraph{Comment 1} 
In Section 5.1 (weak scaling) and 5.2 (strong scaling), the parallel performance of the stable s-step GMRES is compared to the performance of MGS GMRES. It is pretty clear that in this case s-step GMRES is going to win over MGS-GMRES by a wide margin, because MGS-GMRES is probably the most communication-intensive variant of GMRES. Thus, the comparison is unfair. It would be valuable to include either a CGS2-GMRES or one of the low synch variants to make the comparison more meaningful, as CGS2-GMRES requires less communication and in general, is much more favorable in parallel. Also the block orthogonalization in the s-step GMRES is based on CGS2, so comparing the s-step GMRES with CGS2-GMRES would had been justified.

\rpy{See "Response to both reviewers on benchmarking against other algorithms".}

\paragraph{Comment 2}
Also, what polynomial basis was used in parallel experiments? If it was scaled polynomial basis, what was the cost of computing Ritz values?

\rpy{Thank you for your feedback. Yes, scaled Newton polynomial basis is used in all parallel experiments. We have added clarifications in different places of the text to remind readers about this. For instance, see line 731.

The Ritz values are obtained from a standard Arnoldi/GMRES algorithm, so the cost of obtaining the Ritz value would be equivalent to the cost of a standard Arnoldi/GMRES algorithm. As commented at line 341, this is a common strategy in s-step GMRES algorithms. We did not report the cost of this because (a) this can be inferred from the MGS-GMRES results; (b) the cost of obtaining Ritz values can vary depending on the application. For instance, some Ritz values can be known prior to solving the linear system, or when multiple right hand sides are to be solved, the cost of obtaining Ritz value can be amortized. If a standard GMRES algorithm is used to obtain Ritz values, the solution from the GMRES algorithm can also be used as a better initial guess for the s-step GMRES algorithms. In short, the cost of obtaining Ritz values varies depending on the use case and is therefore not included in this manuscript.

In addition to the cost of obtaining Ritz values, there is also some computational cost associated with the incremental condition estimator as well. But as indicated in Equation (3.15), all operations are element-wise operations on a $s\times s$ matrix, which have $O(s^2)$ complxity and typically have negligible computational cost comparing to the GMRES algorithms. In practice, after we obtain the Ritz values, the preprocessing steps for scaled Newton basis with $s = 100$ take about $O(10^{-3})$ seconds in our parallel experiemnts.
}

\paragraph{Comment 3}
All the parallel tests are performed on relatively "easy" problems. It would be valuable to see the performance on a problem that has high condition number, is run to completion (not just for 100 iterations) and (possibly) requires a preconditioner in order to converge. Also it seems like all parallel tests were performed with s=100 and were run for 100 iterations, hence there was no added operations/communication coming from orthogonalization between blocks and restarting GMRES. It would be valuable to see how do these not included operations influence the overall performance, as ideal scenario is unlikely in practice.

\rpy{Thank you for your suggestion. We think this is a great idea. As requested, we have included a set of results in Section 5.2 where a local ILU(0) preconditioner is applied to the Laplace problem and multiple inter-orthogonalization steps are used. See Fig. 14 for the summary of results. 

We acknowledge the importance of using numerically challenging linear systems. However, we chose to use the same Laplace problem due to several reasons. First of all, we want to use a problem with varying dimensions for weak scaling. Weak scaling allows us to demonstrate scalability up to a larger scale, as compared to strong scaling tests which have stringent memory requirements. Weak scaling also allows us to show the timing breakdown clearly. Therefore, we use a PDE problem with varying number of mesh points for weak scaling analysis.

With increasing matrix dimensions, the condition number of the linear system often increases. It becomes increasingly difficult to find an effective preconditioner that accelerates convergence to the same degree and scale well at the same time. Running to completion would mean different (and likely increasing) number of iterations for increasing matrix dimensions. We can definitely fine-tune the preconditioner to reach the same convergence at different matrix sizes, but as our paper focuses on numerical stability instead of accelerating convergence, we feel this is outside the scope of our paper. We also mentioned in Section 2 (line 80) that our work do not aim to optimize the SpMV and preconditioning operations as their communication-avoiding counterparts depend heavily on the sparsity patterns of the matrix and the preconditioner. Hence, in Figure 14, we present a standard local ILU(0) preconditioner for the same 3D Laplace equation without any fine-tuning of the preconditioner. This also allows for reproducibility of the results.

We want to highlight that the initial step size with local ILU(0) preconditioner can be as large as $s=100$ for scaled Newton polynomials in all our tests. But to mimic a numerically challenging problem, we reduced the step size to $s=25$ instead of $s=100$ for the same 100 iterations, so that multiple inter-orthogonalization steps are necessary. In practice, the tests are not fully converged (e.g., $10^{-8}$), but the runtime behavior of the algorithm with additional iterations can be inferred from the current set of results. The results (as presented in Figure 14) can also be compared with the single-block results in Figure 13. 

Overall, we want to provide a set of standard benchmarks with preconditioning steps and inter-orthogonalization steps, and also allow for reproducibility of our results. We hope the arguments above justify the scope of the added tests in Section 5.2.
}

\subsection*{Minor comments}

\paragraph{Comment 1} Line 31-32: "The performance of many operations in Krylov subspace methods, such as dot products and sparse matrix-vector multiplies (SpMVs), is bounded by communication on distributed systems" Consider reformulating - SpMV requires only local communication between (usually neighboring) ranks but dot product requires reduction which leads to global communication - I.e., all ranks communicate partial result and then the full result is distributed. Global communication is what (typically) limits performance in parallel setting.

\rpy{Thank you for your feedback. We agree that global reduction is often what limits performance on large-scale problems. We have updated the text to place emphasize on dot product operations. Please see line 31. }

\paragraph{Comment 2} Line 36: "redesign Krylov subspace methods that communicate less." Either "design Krylov methods that communicate less" or "redesign Krylov methods to communicate less".

\rpy{We have updated the text. Please see line 36.}

\paragraph{Comment 3} Line 40-41:
"BLAS-3 operations that are better optimized for fast memory [19]"
Not clear what "fast memory" means here.

\rpy{By "fast memory", we meant cache memory that allow quick access to data. It has lower latency compared to DRAM. We have updated the text to explicitly mention cache memory. Please see line 41.}

\paragraph{Comment 4} Line 47-48:
"Formulations of s-step Krylov subspace methods are mathematically equivalent to their classical counterparts"
Should probably be: "s-step methods are mathematically equivalent to their classical counterpart" or "s-step method can be formulated/written in such a way that they are mathematically equivalent to their classical counterpart".

\rpy{We have updated the text. Please see line 47.}

\paragraph{Comment 5} Paragraph starting at Line 53: Change "section 2" to "Section 2", "section 3" to "Section 3" etc (section and subsection should be capitalized). "algorithm 2.1" should be "Algorithm 2.1" (please check the entire paper for referencing algorithms and figures - they should be all capitalized).

\rpy{We have updated all references with capitalization. Thank you for your feedback on the format.}

\paragraph{Comment 6} Line 93: "But in finite precision, the Krylov basis vectors converge to the largest eigenvector of matrix A" Should be "eigenvector associated with the largest eigenvalue"

\rpy{We have updated the text for clarification, please see line 94.}

\paragraph{Comment 7} Line 127: "Each block $V^{(i)}$ first needs to be inter-orthogonalized with respect to orthogonal bases generated from previous iterations
[...]"
This statement is unclear; i.e., this is a first time the notion of "iteration" appears in this section. Should probably be $Q^{(1)}$ to $Q^{(I-1)}$ orthogonalized before or similar. Rewrite.

\rpy{We apologize for the ambiguity. We agree it would be best to delay the discussion of "iteration" to later sections. Here, we think it could be more appropriate to use "previous blocks" instead of "previous iterations". Please see line 129 for the updated text.}

\paragraph{Comment 8} Line 128:
"per s vector."
Should be "per s vectors"

\rpy{Thank you for pointing out the typo. We have corrected it in line 141.}

\paragraph{Comment 9} Line 154:
"Here, we note that the input block does not refer to the block $V^{(i)}$"
This statement is unclear I.e., what is $i$?

\rpy{We meant the $i$th block in the original matrix as defined in Equation (2.2). We have updated the text at line 157 to add the reference about Equation (2.2).}

\paragraph{Comment 10} Line 201:
"As mentioned previously, an ill-conditioned input matrix to CholQR may produce a numerically non-SPD Gram matrix"
But from what I understand, the Gram matrix ($V^TV$) IS the input to CholQR. If not, can you specify which Gram matrix are referring to?

\rpy{We apologize for the ambiguity. Here, we treat CholQR as a QR algorithm, so the input is the matrix to be factorized, which is $V$. $V^TV$ is the first computation within the CholQR algorithm. We have added $V$ in the text to further clarify this. Please see line 205. An additional clarification is also included at line 167 where there might be ambiguity.}

\paragraph{Comment 11} Line 209:
$X_{s-p}$ should be of a dimension $[N \times (s-p)]$ not $[n \times (s-p)]$

\rpy{Correct. Thank you for pointing out the typo. We have updated the text at line 212.}.

\paragraph{Comment 12} Line 236:
"that are relatively cheaper"
That are cheaper.

\rpy{We have updated the text. Please see line 239.}

\paragraph{Comment 13} Line 392
"approximate true eigenvalues, we can compute the product term approximately before the actual adaptive s-step GMRES algorithm without any communication cost."
First, in order to use the method, you need Ritz values. And computing them through Arnoldi Gram-Schmidt is not communication free.
Second, what is meant by "the product term"?

\rpy{Thank you for your feedback. We completely agree that computing Ritz values through Arnoldi/GMRES is not communication free and this statement is ambiguous. Here, our intention is to highlight that the initial step size estimator does not add extra communication cost to the original algorithm, which is using scaled Newton polynomials as a basis for adaptive s-step GMRES. 

To further clarify this, we first acknowledge that the construction of scaled Newton polynomial basis, like that of the standard Newton polynomial basis, requires Ritz value computation and is often not communication-free. But the derivations, such as equation (3.14), show that the initial step size estimator only takes in the Rtiz values as input and generates an estimation based on those Ritz values. Since Ritz values are available on all MPI ranks, all the operations in the estimator are done locally to each rank. Hence, the estimator does not incur additional communication cost, which aligns with the objective of communication-avoiding algorithms.

As for the second comment, "the product term" refers to the $\prod_{k=1}^{j-1}{\frac{\lambda_i-\theta_k}{|\bar{\theta}-\theta_k|}}$ in equation (3.14) as indicated by the product operator $\prod$. 

Nonetheless, we added some clarification to the text at line 397-398.
}

\paragraph{Comment 14} Line 415:
"inevitably increases the condition number of the Krylov basis matrix V exponentially."
Rewrite, i.e., "exponential increase in the condition number is inevitable" or similar.

\rpy{We clarified the text. Please refer to line 420.}

\paragraph{Comment 15} Line 434:
"As the Ritz values are available on all processes"
Processors or ranks, not processes.

\rpy{Thank you for your feedback. We updated the text. Please see line 441.}

\paragraph{Comment 16} Line 435:
"the estimator requires no communication cost"
"The estimator requires no communication" or "the estimator incurs no additional communication cost".

\rpy{Thank you. We updated the text. Please see line 441.}

\paragraph{Comment 17} Line 444:
"to verify the implementation sequentially since parallel implementations only introduce additional data movements that do not affect the stability of the overall algorithm."
This is not necessarily true.

\rpy{Yes, we agree this is not technically correct. Roundoff errors can have variations across software/hardwares, and parallelizing a sequential algorithm can potentially introduce these variations in roundoff errors that could modify the stability of the algorithm. However, such consideration is outside the scope of this work and we treat this as an assumption. Please see 450 for clarification.}

\paragraph{Comment 18} Line 461:
"We first start"
We start.

\rpy{Thank you for your feedback. We updated the text. Please see line 467.}

\paragraph{Comment 19} Line 500:
"The periodic pattern of LOO is because"
"The periodic pattern of LOO results from/is a consequence of"

\rpy{Thank you. We have updated the text at line 509.}

\paragraph{Figure 2, Figure 3, Figure 4}
- Use different ticks (i.e. squares, diamonds, circles, triangles, etc) for each quantity so the graphs are easy to understand even if printed in black and white or read by someone with impaired color vision.
- The LOO and convergence curve should be on separate plots.

\rpy{Thank you for your feedback. We have standardized all graphs to include ticks for all curves in the graphs, with appropriate legends. 

As for the second comment, We would like to request to keep it this way for two reasons. The first is that each figure currently consists of multiple sub-figures and is already taking up almost an entire page. Separating LOO and convergence plots will tend to make each figure go out of the scope of a single page. Although we can definitely break them up into two pages, but we feel having one figure per test case on one single page makes each figure more self-contained and helps readers to see the full picture. The second reason is that this arrangement of having LOO and convergence curve in one single plot is consistent with representations in previous literature. E.g., see Figure 2 and 3 in \cite{swirydowicz2020low}, Figure 5 and 6 in \cite{yamazaki2020low}. Nonetheless, we are open to adjusting them if there are strong opinions. To help, we also added a comment at line 479, where we first discuss results using figures, to clarify the content of figures.}

\paragraph{Line 546}
"In practice, especially on large distributed machines, one could use a smaller restart length and more restarts to trade convergence for communication savings."
Smaller restart means more iterations, and more iterations means more communication. Also at the end of each restart, you have an extra norm (which requires a dot product).

\rpy{Thank you for your feedback. We agree with the statement that smaller restart generally means more iterations which in turn implies more communication. However, it is possible to achieve less communication with smaller restarts in certain cases. The statement right after this line (now at line 557) explains such a scenario and we would like to expand on that.

As shown in Fig. 6, for a total of 600 iterations with 4 restarts (restart length = 150), four block iterations are required within each restart (100 + 23 + 23 + 4). Since each block iteration requires 4 global reductions and each restart requires one reduction to compute the norm of residual vectors, a total of $4\times 4 + 1 =17$ global reductions are needed per restart. This leads to a total of $17 \times 4$ = 68 global reductions. If one were to start with a smaller restart length of 100 instead of 150, a total of 6 restarts are required for the same 600 iterations in total. However, each restart of length 100 would only require one block iteration. Hence, the total number of global reductions would be $5\times 6$ = 30, which is fewer than 4 restarts.

We would like to highlight that the algorithm has the flexibility to adjust this restart length on the fly. As mentioned by the statement at line 557, one can start with a restart length of 150. With the adapted step size at $s\approx 100$, the restart length can be adjusted to $s$ for the next restart to reduce the communication costs. The initial step size estimator can also be used as a form of heuristics to inform the restart length. We acknowledge that adjusting restart length will ultimately alter the convergence behavior. Hence, it is a tradeoff between convergence and communication savings and the choice would depend on the actual use case. 

We hope this clarifies that statement. We have also added some clarification in text. See line 560.
}

\paragraph{Line 569}
"rapid growth/decay of Krylov basis vectors."
It should be either condition number or norms, but not vectors.

\rpy{Yes, we meant the condition numbers of Krylov basis vectors. We have clarified at line 582.}

\paragraph{Line 679} "growth starts depends"
Starts depending

\rpy{Grammatically we think the original text is correct. We meant the exact column (...) depends on the eigenvalue spectrum. Please see the statement currently at line 692.}

\paragraph{Line 717}
"done on Intel Xeon Platinum 8280 processors with 56 cores"
It is clear from the results that not one processor, but entire cluster of them was used. More details of hardware are needed. Also the details of software (version of compiler and libraries used) should be given for reproducibility.

\rpy{Thank you for pointing out this. We apologize for the ambiguity. We have added two short paragraphs at line 762-779 about both the software and hardware used in the parallel experiments.}

\paragraph{Line 754}
"MPK that can explore efficient fast memory usage."
This is a vague statement - please expand.

\rpy{We observed that the MPK kernel in adaptive s-step GMRES, which consists of consecutive SpMVs, is slightly faster than the standard SpMVs that are called at each iteration of MGS-GMRES. Both the MPK kernel in s-step GMRES and SpMVs in MGS-GMRES have approximately the same amount of floating point operators and communication costs. The main difference is that in MPK kernels, SpMVs are called repetitively before any orthogonalization. We want to highlight that we do not make any modification to SpMV kernels. We use the built-in SpMV available in PETSc. We simply call them multiple times in a MPK kernel (with some \texttt{axpy} vector operations for basis computation). Hence, they are essentially the same function calls, but in a different order. Hence, we conjectured that the small difference in performance of MPK/SpMV kernels is because compiler was able to optimize MPK better than standard SpMVs by exploring cache memory. For instance, in MPK, consecutive SpMVs allows the matrix (or part of it) to stay in cache longer for efficient computation. 

Due to the rewrite of results section, we have paraphrased the text with additional details. Please see the paragraph at line 825.}


==> Review/reviewer1_round2.tex <==
\section*{Response to reviewer \#1}
\rpy{(Responses are highlighted in red. Corresponding code changes are highlighted in red as well in the manuscript.)}

\subsection*{Minor comments}
\paragraph{Comment 1} 
Please fix hyperlinks. For instance, when I click on Algorithm 2.2 (line 205), the hyperlink takes me to the first page. Similar with other links in the text. Probably simple LaTeX error/compilation issue.

\rpy{Thank you for bringing this to our attention. We believe this is indeed a technical error due to an erroneous LaTex command. We have corrected it and generated a new PDF with correct hyperlinks.}


\paragraph{Comment 2} 
Line 72: "At each iteration, the Matrix Powers Kernel (MPK) performs s SpMVs on a starting normalized column vector $Q_i$" -- unclear what $i$ is/ Consider adding "at step/iteration/block iteration $i$"

\rpy{Thank you for your feedback. We have added the clarification at line 72}


\paragraph{Comment 3} 
Line 152: "Barlow showed that BCGS2 produce " $\rightarrow$ "Barlow showed that BCGS2 produces"

\rpy{Thank you for your feedback. We have corrected the typo at line 152}


\paragraph{Comment 4} 
Line 167: capitalize Algorithm.

Line 205: capitalize Algorithm.

\rpy{Thank you for your feedback. We have corrected the typo at line 167 and 205.}


\paragraph{Comment 5 (Series of comments about mismatching figure numbers)} 
Line 477: It should probably be Fig 2, not Fig 3 (Fig 3 is for 2D Laplace). Same in Line 490.

Line508: It should be Fig 3 not Fig 4. 

Line525: Should be Fig 4, not Fig 5 (based on figure captions). Same in Line 532.

Line540: Should be Fig 5, not Fig 6. Same comment, Line 560.

Line599: Should be Fig 6, not Fig 7. Also line 600 should be Fig 5.

Line607: Should be Fig 7.

Line623: Should be Fig 7.

Line642: Fig 8, not Fig 9.

Line652: Fig 9, not Fig 10.

Line664: Fig 10, not Fig 11.

Line684: Fig 10, not Fig 11.

Line699: Fig 10, not Fig 11. Also check line 703 for correct figure references.

Line718: Fig 11, not Fig 12.

Line794: Fig 12, not Fig 13. Also Line 826.

Line846: Fig 12, not Fig 13.

Line909: Fig 13, not Fig 14. Same in Lines 909, 910, 918.

Line934: Should be Fig 14, not Fig 15.

Line 935: Fig 15, not Fig 16.

Line 959: Fig 15, not FIg 16.

\rpy{Thank you for your feedback about the wrong numbering of figures and we appreciate the detailed tracking of all the wrong numbering of references. This issue was also raised by another referee. The wrong numbering has been tracked down to an erroneous LaTex command in the previous manuscript that incorrectly incremented the numbering of all figure references by 1. In other words, all references to Figure $x$ were incorrectly compiled to Figure $x+1$ in text. We apologize for the technical error. This has been fixed in the revised manuscript.}


\paragraph{Comment 6} 
Figure 11: Some matrices used are symmetric positive definite (say Thermal2) and CG can be applied (GMRES is an overkill). Others (say Delaunay\_n20, belgium\_osm) are not linear system matrices. Maybe justify your choice in the caption?

\rpy{Thank you for pointing this out. We believe there are two parts to the question here, one regarding symmetric positive definite (SPD) matrices and the other about non-linear system matrices.

Our original intention was to randomly choose several large-scale matrices ($N>10^6$) from SuiteSparse Matrix Collection for testing. During the selection process, we did not explicitly exclude SPD matrices. Although our paper is on GMRES variants, this particular section on initial step size estimator could potentially apply to adaptive s-step CG for SPD matrices since the estimator only relies on the eigenvalue distributions. For this reason, in the revised manuscript, we have 2 SPD matrices in the selection (\texttt{G3\_circuit} and \texttt{thermal2}).

On the other hand, we did make the careless mistake of including matrices that are not really linear system matrices. This was tracked down to a careless selection on the SuiteSparse website where we did not filter the field \textit{Rutherford-Boeing Type} so that binary matrices were included. This has been corrected in the revised manuscript where binary matrices are removed and only real matrices are included. We have also added additional matrices to demonstrate the robustness of our proposed estimator.

To clarify the selection of matrices, we have included a table (Table. 1) in \textit{Section 4, Test 10} to display the vast range of domains that we have tested our algorithm on. All matrices are of size $N>10^6$.}


\paragraph{Comment 7} 
Line 648: "The E20R5000 matrix with the ILU(0) preconditioner does not converge well" $\rightarrow$ it is not the matrix that converges, but the linear system with the matrix.

\rpy{Thank you for your feedback. We have added the clarification at line 645 about the linear system.}


\paragraph{Comment 8} 
Line 508: Also, in the caption of Fig 4, the size is 1.6*$10^6$ while in the text it is 1.6 * $10^5$.

\rpy{Thank you for your feedback. The correct dimension is $1.6\times10^5$ as it is generated from a $400\times 400$ 2D mesh. We have corrected the typo in the caption of Figure 4.}


\paragraph{Comment 9} 
Line 636: "Test 6: 2DLaplace" -> "Test 6: 2D Laplace" (missing space).

\rpy{Thank you for your feedback. We have corrected the typo in the parapraph header at line 633.}


\paragraph{Comment 10} 
Reference [39]: fix capitalization.

\rpy{Thank you for your feedback. We have fixed the capitalization. We also removed a redundant bibliography entry during our proofreading. The original reference [39] is now [38].}

==> Review/reviewer2.tex <==
\newpage
\section*{Response to reviewer \#2}
\rpy{(Responses are highlighted in red. Corresponding code changes are highlighted in red as well in the manuscript.)}

\subsection*{Major comments}
\paragraph{Comment 1} 
The first is not comparing to s-step GMRES using TSQR, as in [23,28]. The authors say that part of their motivation is fixing the LOO (loss of orthogonality) from doing Cholesky QR (CholQR) to compute an orthogonal basis of the desired Krylov subspace. But TSQR is guaranteed to provide an orthogonal basis, and also avoid communication. And the incremental condition estimation (ICE) proposed by the authors to choose which leading columns of the R factor are sufficiently well conditioned still applies. This could also be used to reduce the cost of reconstructing (a subset of) the Q factor.

\rpy{See "Response to both reviewers on benchmarking against other algorithms".}

The second omitted observation is in the paper “Theory of inexact Krylov Subspace methods and applications to scientific computing,” V. Simoncini and D. Szyld, SISC, 2003, cited in [10].
Rather than have the adaptive step size s remain constant throughout the iterations, Simoncini and Szyld show that you can relax the accuracy of the SpMV at a rate inversely proportional to the residual norm. The translation of this to s-step CG in [10] was that you could start off with a smaller s (when the residual is large) and make s larger and larger as the residual converges without losing accuracy. The work of Simoncini and Szyld certainly applies to GMRES (arguably more so than CG), so I don’t see why a similar principle shouldn’t hold for s-step GMRES. Perhaps the use of CholQR instead of TSQR limits s further?

\rpy{We appreciate your comment. This is a very good point. We did study the s-step CG work in [11] in detail and have commented on its difference from our method in Subsection 2.3. We are also aware of the work of inexact Krylov subspace methods. But we do not apply them directly in our work for three reasons.
\begin{itemize}
\item The mathematical derivation in section 4.1 in [11] shows a direct relationship between the residual and the condition number of the Krylov basis matrix in the s-step CG method. The relationship indicates one can relax the constraint on condition number of the Krylov basis matrix. However, such a relationship is not mathematically derived in this work due to the complexity of the block QR algorithms. As repetitively emphasized in this work, the key challenges in an s-step GMRES algorithm lies in the numerical stability of the block QR algorithm. There are many different choices for inter-orthogonalization and intra-orthogonalization. The backward stability of many block QR algorithms is still largely an open problem, as pointed out by [9]. It is not clear to us if a simple relation like equation (4.13) in [11] has its equivalent form in the s-step GMRES algorithm, given the wide range of choices of block QR algorithms. In this work, we focus on numerical experiments to empirically verify the numerical stability of the proposed algorithm. Hence, we did not attempt such a mathematical derivation for the our s-step GMRES algorithm. This could be an extension for future work.
\item From a practical standpoint, we did not find this method of increasing $s$ to be efficient in our framework. In the s-step CG method proposed in [11], all tests were carried out using monomials (see Section 5 of [11]) where Ritz values are not required. Hence, increasing $s$ on the fly through relaxation does not incur additional costs. In our framework, we have demonstrated the benefit of using scaled Newton polynomial to significantly increase the step size to $O(100)$ and it is important that Ritz values are pre-computed to set up the Newton polynomial basis. In practice, with an initial step size of $s_0$, only $s_0$ Ritz values are pre-computed. Allowing the step size to increase beyond $s_0$ through some form of relaxation will require additional Ritz value computation that incur additional (both computational and communication) costs. 
\item If the adapted step size is smaller than $s_0$, we could potentially increase the step size in subsequent block iterations as long as it stays below $s_0$ so that we do not have to compute additional Ritz values. However, empirically we do not observe such an increase in adapted step size in consecutive block iterations. For instance, in Fig. 6, 7 and 10, the step size decreases rapidly after the first block iteration. Without deriving the exact mathematical relationship, we conjecture this is due to the fact that subsequent block iterations are trying to construct a set of orthogonal basis in a smaller subspace that has to be orthogonal to the subspace spanned by the Krylov basis in previous blocks. Therefore, it could be numerically challenging to retain a very large step size as the block iteration continues.
In addition, the lower two figures of Fig. 6 indicate that the condition number of the Krylov basis matrix can change significantly after an inter-orthogonalization step. These observations do not seem to imply a direct relationship between the condition number of Krylov basis vector and the solution residual, in the form of equation (4.13) in [11]. Even with TSQR as an intra-orthogonalization scheme, the exponential increase in condition number of block $R(1:j,1:j)$ in Fig. 6 does not seem to suggest that TSQR could increase the step size significantly. 
\end{itemize}
In summary, given the complexity of block QR algorithms in s-step GMRES, we feel that the derivation of a mathematical expression relating the residual and adapted step size to be outside the scope of this work. Without a detailed derivation, we do not find strong empirical evidence that increasing the step size via the theory of inexact Krylov subspace could benefit the overall framework of our proposed algorithm. However, we recognize the significance of inexact Krylov subspace methods and are happy to discuss potential avenues for addressing this in future studies.

}

\subsection*{Minor comments}

\paragraph{Comment 1} Algorithm 2.2, which is called in Algorithm 2.1, repeat the calling sequence to make it easier to match variable names with Algorithm 2.1.

\rpy{Thank you for the feedback. We totally agree and have added the calling in Algorithm 2.2.}

\paragraph{Comment 2} Line 412: Change ”for arbitrary starting vector” to ”for an arbitrary starting vector”.

\rpy{Thank you for pointing out the typo. We have corrected it at line 417.}

\paragraph{Comment 3} Line 421: Change $E_{i,j}\in \mathbb{R}^{s\times s}$ to $E\in \mathbb{R}^{s\times s}$, for consistency with equation (3.15).

\rpy{We are slightly confused as equation (3.15) is defined using $E_{i,j}\in \mathbb{R}^{s\times s}$ which is consistent with the text. Please see line 427. We would appreciate if the reviewer can elaborate on this comment.}

\paragraph{Comment 4} In Fig 2 (and later figures), the same labeling (black circles or red diamonds) is used for 2 curves with 2 meanings, which makes it difficult for the reader to tell which is which. Also, in the caption, the phrase ”The LOO of the algorithm” is ambiguous as to which algorithm it refers to, be explicit.

\rpy{Thank you for the feedback. The two curves are implicitly differentiated via where they start and how they progress. The relative residuals start from 1 and gradually decrease, where indicate convergence of the various GMRES algorithm. The loss of orthogonality (LOO) error curves start from machine epsilon, gradually increase and their rates of increase reflect the accuracy of the orthogonalization schemes in each GMRES variant. This is consistent with representations in previous literature. E.g., see Figure 2 and 3 in [34], Figure 5 and 6 in [38]. Nonetheless, we added some clarification at line 479 where we first discuss results using figures. We also updated the captions in multiple figures.}

\paragraph{Comment 5} Line 536: The notation $\kappa(V_{1:j,1:j})$ seems wrong, since all rows of the tall matrix V should be included.

\rpy{Thank you for pointing out the typo. Yes, we agree this should be $\kappa(V_{:,1:j})$ and we have updated both the text at line 546 and the figure label in Fig. 6.}

\paragraph{Comment 6} References: there are many capitalization errors, eg gmres instead of GMRES, etc.

\rpy{Thank you for pointing it out. We apologize for the formatting error. We made a Latex mistake which led to capitalization inconsistencies. We have corrected the capitalization error and updated the reference.}

==> Review/reviewer2_round2.tex <==
\newpage
\section*{Response to reviewer \#2}
\rpy{(Responses are highlighted in red. Corresponding code changes are highlighted in red as well in the manuscript.)}

\subsection*{Major comments}
\paragraph{Comment 1} 
This revision addresses most of my comments in my previous review. I have one more mathe- matical question, and some minor editing suggestions.

The mathematical question is regarding the implementation of BCGS2-TSQR-GMRES in section 5. It is possible to implement GMRES without computing the explicit columns of the Q matrix, since we only need to multiply by Q or $Q^T$ , which can be cheaper for TSQR. Does the authors’ implementation take advantage of this optimization, or do they form Q explicitly? Either way, they should document this.

\rpy{Thank you for raising this question. This is indeed a very intriguing question. For discussion purposes, we would like to first establish the notation and concepts regarding implicit Q factor in TSQR. Here, we borrowing the notation in [19] where a matrix $A$ can be factorized using TSQR as (Equation 1 in Section 4.1 of [19]):

\[
A = \begin{pmatrix}
A_0 \\ 
A_1 \\ 
A_2 \\ 
A_3
\end{pmatrix} 
= \left( \begin{array}{cccc}
Q_{00} & & & \\
 & Q_{10} & & \\
 & & Q_{20} & \\
 & & & Q_{30}
\end{array} \right)
\cdot \left( \begin{array}{cc}
Q_{01} & \\
 & Q_{11}
\end{array} \right) 
\cdot Q_{02} \cdot R_{02}
\]

(We only show 3 stages as an illustration.) The final Q factor is a product of all the $Q_{ij}$ matrices. Instead of computing the $Q$ factor explicitly, all operations involving multiplying by $Q$ or $Q^T$ can be achieved by multiplying the $Q_{ij}$ factors implicitly. The action of explictly computing the $Q$ factor from $Q_{ij}$ incurs the same communication cost (same number of messages) as applying $Q$ or $Q^T$ to a vector. The communication pattern is akin to a broadcast operation (with custom communication tree pattern).

In this work, our original implementation of TSQR was using the \textbf{explicit} $Q$ factorization where we explicitly compute the $Q$ matrix and store it. This is largely because we implemented the TSQR algorithm using the \texttt{SLEPC} library and the implementation in \texttt{SLEPC} provides only explicit $Q$ factorization. For reproducibility, we did not modify the implementation in \texttt{SLEPC}.

Regarding the implicit version, we find that the use of implicit representation of $Q$ factor is indeed possible since we do not actually require explicit entries of the $Q$ factor. But whether the implicit representation brings any performance gain is worth some in-depth discussion. This is mostly because that the \textit{intra-orthogonalization} TSQR kernel needs to be evaluated in the context of block QR scheme where TSQR needs to be coupled with the \textit{inter-orthogonalization} scheme BCGS2. We feel the performance is largely dependent on the implementation. To elaborate on this, we summarize the BCGS2\-TSQR\-GMRES alrogithm below as a block QR algorithm:
\begin{algorithm}
\caption{Block QR using BCGS2 and TSQR}
\begin{algorithmic}[1]
\REQUIRE Step size \textit{s}, index $i$, Krylov basis matrix $V$ of size $N\times s$, orthogonal basis matrix $Q_{1:i}$ of size $N\times i$.
\ENSURE Orthogonal basis matrix $Q_{i+1:i+s}$ of size $N\times s$, upper triangular matrix $R_{1:i+s,i+1:i+s}$ of size $(i+1) \times s$.
\STATE $k = i+1:i+s$
\STATE
\STATE $W = Q_{1:i}^TV$ \COMMENT{First BCGS}
\STATE $V = V- Q_{1:i}W$
\STATE $[\,Q_{k},\, Z\,] = \mbox{TSQR}(V^TV, \Omega)$ \COMMENT{First TSQR}
\STATE
\STATE $R_{1:i, k} = Q_{1:i}^TQ_{k}$ \COMMENT{Second BCGS}
\STATE $Q_{k} = Q_{k} - Q_{1:i}R_{1:i, k}$
\STATE $[\,Q_{k},\, \tilde{Z}\,] = \mbox{TSQR}(Q_{k}^TQ_{k}, \Omega)$ \COMMENT{Second TSQR}
\STATE
\STATE $R_{1:i, } = W_{:,1:s} + R_{1:i, k}Z$ \COMMENT{Combine both steps}
\STATE $R_{k, k} = \tilde{Z}Z$
\end{algorithmic}
\end{algorithm}
Here, we have replaced the Partial CholQR in Algorithm 3.2 with TSQR. We assume the adaptive step size is exactly $s$ (i.e., no truncation) to simplify the discussion. (The adaptive nature of Partial CholQR can be easily enabled via a condition number estimator after each TSQR.) At each TSQR stage, the $Q_k$ factor can be implicitly constructed as a product of multiple $Q_{ij}$ matrices (with some abuse of notation here). 

We investigate the trade-offs between using implicit and explicit $Q$ representations from a few aspects.
\begin{enumerate}
	\item For the first TSQR, if the $Q_k$ matrix is expressed implicitly. The second step of BCGS needs to be adjusted since it does require an update to the $Q_k$ matrix (at line 8 of the above algorithm). It is possible to use an implicit representation of $Q_k$ and store the product of $Q_{1:i}R_{1:i, k}$ first, then later compute the $Q_{k}^TQ_{k}$ matrix at line 9 via factorization (i.e., $(Q_{k} - Q_{1:i}R_{1:i, k})^T(Q_{k} - Q_{1:i}R_{1:i, k})$). However, this incurs additional storage cost for the term $Q_{1:i}R_{1:i, k}$. With explicit representation of $Q_k$, it is almost trivial to implement the second BCGS and we only need to store the $Q_k$ matrix itself without the need to store other auxiliary $Q_{ij}$ matrices. 
	\item In terms of communication cost, although implicit representation of $Q_k$ factor saves a communication step that is similar to a broadcast operation within the TSQR kernel, we still need to apply the orthogonal matrix at line 8 and 9 in the second BCGS step. Hence, the number of messages sent is the same as the explicit representation. The latency cost also stays relatively at the same order since TSQR kernel still requires a global communication call to compute the $R$ factor.
	\item As we have demonstrated in the Weak Scaling results (Fig. 12), the efficient utilization of BLAS-3 kernels is crucial in achieving good performance on the hardware. Using explicit $Q$ representation has the advantage to fully leverage high-optimized BLAS-3 kernels provided by software vendors/developers. Implicit $Q$ representation requires multiplication of small-scale $Q_{ij}$ matrices that might hinder the optimization provided by BLAS-3 libraries.
	\item As our algorithm adaptively selects the number of the orthogonal bases at each block iteration, truncation of irrelevant orthogonal bases can be done efficiently if the $Q$ matrix is represently explicitly. For instance, with an initial step size of $s_0$ and an adaptive step size of $s^*$, truncation of orthogonal basis vectors means $s_0 - s^*$ column vectors can be removed from storage. With implicit representation, this is non-trivial as only the last $Q_{ij}$ matrix can be truncated, while $Q_{i0}$ would still have to contain the entire $s_0$ column vectors.
\end{enumerate}

In summary, the use of implicit $Q$ representation is allowed for the adaptive $s$-step algorithm, but the potential savings acheived by implicit $Q$ representation has to be balanced off by efficient implementation of the related kernels. As the exact software implementation of optimized kernels for TSQR is outside the scope of this work, we would like leave this pursuit of implicit $Q$ version of TSQR in adaptive $s$-step GMRES as future work. Nonetheless, we have added clarification in Section 5 (line 765).
}

\subsection*{Minor comments}

\paragraph{Comment 1}
1. Page 12, line 400: The reference to Fig. 2 should be to Fig. 1. All later references to figures in the text seem to be off-by-one as well.

\rpy{Thank you for your feedback about the wrong numbering of figures. This was similarly pointed out by the other referee. The numbering mistake has been tracked down to an erroneous LaTex command in the previous manuscript, which incorrectly incremented the numbering of all figure references by 1. In other words, all references to Figure $x$ were incorrectly compiled to Figure $x+1$ in text. We apologize for the technical error. This has been fixed in the revised manuscript.}

\paragraph{Comment 2}
2. Page 18, line 562: “restart cycle” should be “restart cycles”.

\rpy{Thank you for your feedback. We have corrected the typo at line 559}

\paragraph{Comment 3}
3. Page 21, line 641: When the ILU preconditioner is used, how were the rows and columns ordered, since this could impact convergence? The same question applies to other uses of ILU.

\rpy{We would like to first clarify that the rows and columns are not ordered before solving the linear system. For ILUTP though, pivoting is used to assist in accelerating convergence. 

We would also like to re-iterate that the goal of our algorithm (adaptive s-step GMRES) is to acheive the same level of accuracy as the conventional GMRES with minimal communication costs. Hence, the purpose of these tests is to demonstrate the agreement with GMRES under different scenarios. We acknowledge that using ordering could potentially accelerate convergence, but we do not spend effort on tuning the preconditioner for the best possible convergence acceleration since that's outside the scope of this work. 
}

\paragraph{Comment 4}
4. Page 29, line 785: “$16B \times 10^9$” should probably be “$16 \times 10^9$”.

\rpy{Thank you for your feedback. We have corrected the typo at line 777}

\paragraph{Comment 5}
5. Page 30, caption for Figure 12: Describing the timing as SpMV/MPK as “inverted”, which presumably means appearing as negative values below the 0 line, is confusing. This should be explained more clearly.

\rpy{Thank you for your feedback. The SpMV/MPK timing is shown below the x-axis to separate it from the timing of Orthogonalization steps. This is to avoid stacking all timings together and to help readers to visually observe the scalability of each compoenent. We have added some clarification in the caption to explain this.}

\paragraph{Comment 6}
6. Page 30, line 849: The phrase “exponential increase” appears to refer to going from O(s) to O($s^2$), which is only polynomial, not exponential.

\rpy{Thank you for your feedback. We agree the use of 'exponential increase' is technically incorrect and it should be polynomial. We have corrected the typo at line 813.}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
